Search for High-Mass Resonances Decaying to $\tau\nu$ in $pp$ Collisions at $\sqrt{s}$ = 13 TeV with the ATLAS Detector

A search for high-mass resonances decaying to $\tau\nu$ using proton-proton collisions at $\sqrt{s}$ = 13 TeV produced by the Large Hadron Collider is presented. Only $\tau$-lepton decays with hadrons in the final state are considered. The data were recorded with the ATLAS detector and correspond to an integrated luminosity of 36.1 fb$^{-1}$. No statistically significant excess above the Standard Model expectation is observed; model-independent upper limits are set on the visible $\tau\nu$ production cross section. Heavy $W^{\prime}$ bosons with masses less than 3.7 TeV in the Sequential Standard Model and masses less than 2.2-3.8 TeV depending on the coupling in the non-universal G(221) model are excluded at the 95% credibility level.

==> Acknowledgements.tex <==
% Acknowledgements for papers with collision data
% Version 14-Feb-2018

% Standard acknowledgements start here
%----------------------------------------------
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC, Australia; BMWFW and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP, Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic; DNRF and DNSRC, Denmark; IN2P3-CNRS, CEA-DRF/IRFU, France; SRNSFG, Georgia; BMBF, HGF, and MPG, Germany; GSRT, Greece; RGC, Hong Kong SAR, China; ISF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; NWO, Netherlands; RCN, Norway; MNiSW and NCN, Poland; FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MESTD, Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa; MINECO, Spain; SRC and Wallenberg Foundation, Sweden; SERI, SNSF and Cantons of Bern and Geneva, Switzerland; MOST, Taiwan; TAEK, Turkey; STFC, United Kingdom; DOE and NSF, United States of America. In addition, individual groups and members have received support from BCKDF, the Canada Council, CANARIE, CRC, Compute Canada, FQRNT, and the Ontario Innovation Trust, Canada; EPLANET, ERC, ERDF, FP7, Horizon 2020 and Marie Sk{\l}odowska-Curie Actions, European Union; Investissements d'Avenir Labex and Idex, ANR, R{\'e}gion Auvergne and Fondation Partager le Savoir, France; DFG and AvH Foundation, Germany; Herakleitos, Thales and Aristeia programmes co-financed by EU-ESF and the Greek NSRF; BSF, GIF and Minerva, Israel; BRF, Norway; CERCA Programme Generalitat de Catalunya, Generalitat Valenciana, Spain; the Royal Society and Leverhulme Trust, United Kingdom.

The crucial computing support from all WLCG partners is acknowledged gratefully, in particular from CERN, the ATLAS Tier-1 facilities at TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France), KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain), ASGC (Taiwan), RAL (UK) and BNL (USA), the Tier-2 facilities worldwide and large non-WLCG resource providers. Major contributors of computing resources are listed in Ref.~\cite{ATL-GEN-PUB-2016-002}.
%----------------------------------------------



==> EXOT-2017-06-PAPER-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
%\AtlasTitle{A search for high-mass resonances decaying to $\tau\nu$ in $pp$ collisions at $\sqrt{s}=\SI{13}{\TeV}$ with the ATLAS detector}
\AtlasTitle{Search for High-Mass Resonances Decaying to $\tau\nu$ in $pp$ Collisions at $\sqrt{s}=\SI{13}{\TeV}$ with the ATLAS Detector}

%\AtlasVersion{2.5}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%

A search for high-mass resonances decaying to $\tau\nu$ using proton--proton
collisions at \mbox{$\sqrt{s}=\SI{13}{\TeV}$} produced by the Large Hadron
Collider is presented.  Only $\tau$-lepton decays with hadrons in the 
final state are considered.  The data were recorded with the ATLAS detector and correspond to
an integrated luminosity of \SI{36.1}{\ifb}.  No statistically significant
excess above the Standard Model expectation is observed; model-independent
upper limits are set on the visible $\tau\nu$ production cross section.
Heavy $W^{\prime}$ bosons with masses less than \SI{3.7}{\TeV} in the Sequential
Standard Model and masses less than \mbox{2.2--\SI{3.8}{\TeV}} depending on
the coupling in the non-universal $G(221)$ model are excluded at the 95\%
credibility level. 

}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{EXOT-2017-06}

% CERN preprint number
\PreprintIdNumber{CERN-EP-2017-341}

% ATLAS date - arXiv submission; usually filled in by the Physics Office
% \AtlasDate{\today}

% ATLAS heading - heading at top of title page. Set for TDR etc.
% \AtlasHeading{ATLAS ABC TDR}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
%\AtlasJournal{Phys.\ Lett.\ B.}
\AtlasJournal{Phys. Rev. Lett.}
\AtlasJournalRef{\PRL120 (2018) 161802}
\AtlasDOI{10.1103/PhysRevLett.120.161802}

